Characterizing the population of pulsars in the inner Galaxy with the Fermi Large Area Telescope

An excess of $\gamma$-ray emission from the Galactic Center (GC) region with respect to predictions based on a variety of interstellar emission models and $\gamma$-ray source catalogs has been found by many groups using data from the {\it Fermi} Large Area Telescope (LAT). Several interpretations of this excess have been invoked. In this paper we search for members of an unresolved population of $\gamma$-ray pulsars located in the inner Galaxy that are predicted by the interpretation of the GC excess as being due to a population of such sources. We use cataloged LAT sources to derive criteria that efficiently select pulsars with very small contamination from blazars. We search for point sources in the inner $40^\circ\times40^\circ$ region of the Galaxy, derive a list of approximately 400 sources, and apply pulsar selection criteria to extract pulsar candidates among our source list. We performed the entire data analysis chain with two different interstellar emission models (IEMs), and found a total of 135 pulsar candidates, of which 66 were selected with both IEMs.

==> app_tables.tex <==
\begin{table*}
\center
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Name & l[deg]& b[deg] & pos\_68 & $TS$  & $TS^{\rm{PLE}}_{\rm{curv}}$  & $S$[$10^{-5}$MeV/cm$^2$/s] & $\Gamma$ & $E_{\rm{cutoff}}$ & IEM\\
\hline
\hline
 3FGL J1730.6-0357 & 19.72 & 16.00 & 0.02 & 254.0 & 34.9 & $0.39\pm0.04$ & $0.62\pm0.52$ & $1.46\pm0.49$ & Alt./Off.\\
\hline 
 PS J1727.2-0723 & 16.29 & 15.01 & 0.10 & 29.4 & 17.6 & $0.10\pm0.03$ & $1.32\pm0.68$ & $0.84\pm0.12$ & Alt./Off.\\
\hline 
 3FGL J1804.5-0850 & 19.62 & 6.25 & 0.03 & 75.8 & 24.5 & $0.24\pm0.04$ & $0.90\pm0.53$ & $4.37\pm1.90$ & Alt./Off.\\
\hline 
 3FGL J1820.3-1529c & 15.69 & -0.30 & 0.06 & 165.8 & 90.7 & $1.33\pm0.20$ & $1.10\pm0.60$ & $1.17\pm0.43$ & Alt./Off.\\
\hline 
 PS J1827.9-1137 & 19.94 & -0.15 & 0.05 & 36.0 & 11.0 & $0.43\pm0.10$ & $0.49\pm0.34$ & $1.06\pm0.54$ & Alt./Off.\\
\hline 
 3FGL J1830.7-1630 & 15.85 & -3.03 & 0.02 & 226.6 & 174.4 & $0.56\pm0.06$ & $1.25\pm0.27$ & $4.21\pm1.33$ & Alt./Off.\\
\hline 
 PS J1905.9-1718 & 18.92 & -10.91 & 0.08 & 36.1 & 16.7 & $0.08\pm0.02$ & $0.45\pm0.38$ & $0.87\pm0.25$ & Alt./Off.\\
\hline 
 PS J1906.5-1755 & 18.44 & -11.30 & 0.06 & 53.1 & 13.8 & $0.10\pm0.02$ & $0.79\pm0.61$ & $0.81\pm0.45$ & Alt./Off.\\
\hline 
 3FGL J1709.4-0917 & 12.45 & 17.70 & 0.06 & 66.4 & 10.3 & $0.24\pm0.04$ & $1.51\pm0.62$ & $2.03\pm1.48$ & Alt./Off.\\
\hline 
 3FGL J1743.9-1310 & 13.34 & 8.45 & 0.03 & 115.7 & 21.1 & $0.30\pm0.04$ & $1.12\pm0.43$ & $3.39\pm1.54$ & Alt./Off.\\
\hline 
 3FGL J1744.8-1557 & 11.02 & 6.90 & 0.05 & 74.3 & 21.4 & $0.21\pm0.04$ & $0.06\pm0.95$ & $1.33\pm0.64$ & Alt./Off.\\
\hline 
 3FGL J1814.1-1734c & 13.08 & -0.03 & 0.04 & 116.5 & 87.4 & $1.12\pm0.25$ & $0.90\pm0.80$ & $1.51\pm0.79$ & Alt./Off.\\
\hline 
 PS J1807.6-2025 & 9.85 & -0.04 & 0.05 & 85.6 & 75.8 & $0.94\pm0.19$ & $1.09\pm0.86$ & $1.28\pm0.76$ & Alt./Off.\\
\hline 
 PS J1807.1-2114 & 8.95 & -0.27 & 0.04 & 195.5 & 44.6 & $1.54\pm0.23$ & $1.32\pm0.45$ & $1.81\pm0.66$ & Alt./Off.\\
\hline 
 PS J1830.9-2416 & 8.97 & -6.58 & 0.09 & 26.3 & 10.8 & $0.11\pm0.03$ & $0.11\pm0.33$ & $1.34\pm1.15$ & Alt./Off.\\
\hline 
 3FGL J1845.5-2524 & 9.51 & -10.14 & 0.04 & 117.4 & 14.3 & $0.29\pm0.04$ & $1.68\pm0.32$ & $4.59\pm2.24$ & Alt./Off.\\
\hline 
 PS J1909.6-2515 & 11.87 & -15.02 & 0.16 & 25.1 & 15.0 & $0.07\pm0.02$ & $1.90\pm0.23$ & $0.42\pm0.07$ & Alt./Off.\\
\hline 
 PS J1659.2-1445 & 5.96 & 16.79 & 0.05 & 67.0 & 12.5 & $0.18\pm0.03$ & $0.78\pm0.70$ & $2.01\pm1.09$ & Alt./Off.\\
\hline 
 3FGL J1759.6-2141 & 7.85 & 0.95 & 0.03 & 152.4 & 2011.7 & $0.89\pm0.10$ & $1.89\pm0.22$ & $6.81\pm2.84$ & Alt./Off.\\
\hline 
 3FGL J1758.8-2402 & 5.72 & -0.04 & 0.03 & 252.6 & 149.4 & $1.63\pm0.16$ & $1.66\pm0.19$ & $7.13\pm2.64$ & Alt./Off.\\
\hline 
 PS J1756.1-2516 & 4.35 & -0.11 & 0.07 & 88.3 & 30.3 & $0.75\pm0.12$ & $0.84\pm0.88$ & $1.93\pm1.61$ & Alt./Off.\\
\hline 
 3FGL J1816.2-2726 & 4.67 & -4.95 & 0.06 & 76.2 & 18.4 & $0.29\pm0.04$ & $1.78\pm0.32$ & $5.99\pm3.55$ & Alt./Off.\\
\hline 
 PS J1835.0-2817 & 5.75 & -9.20 & 0.06 & 33.8 & 12.6 & $0.12\pm0.03$ & $1.00\pm0.73$ & $3.04\pm1.76$ & Alt./Off.\\
\hline 
 3FGL J1917.1-3024 & 7.53 & -18.41 & 0.02 & 289.9 & 28.5 & $0.35\pm0.03$ & $1.24\pm0.24$ & $5.40\pm1.73$ & Alt./Off.\\
\hline 
 PS J1917.6-3206 & 5.94 & -19.17 & 0.07 & 52.1 & 12.7 & $0.12\pm0.02$ & $0.62\pm0.76$ & $1.21\pm0.83$ & Alt./Off.\\
\hline 
 PS J1711.8-1922 & 3.85 & 11.67 & 0.03 & 96.7 & 22.9 & $0.18\pm0.03$ & $0.69\pm0.49$ & $3.10\pm1.21$ & Alt./Off.\\
\hline 
 PS J1727.8-2305 & 2.80 & 6.53 & 0.04 & 45.6 & 12.7 & $0.16\pm0.04$ & $0.56\pm0.64$ & $4.93\pm2.31$ & Alt./Off.\\
\hline 
 3FGL J1740.5-2726 & 0.68 & 1.73 & 0.03 & 180.8 & 20.6 & $0.94\pm0.21$ & $1.73\pm1.03$ & $1.73\pm1.03$ & Alt./Off.\\
\hline 
 3FGL J1754.0-2538 & 3.77 & 0.11 & 0.01 & 763.3 & 139.3 & $2.18\pm0.12$ & $1.08\pm0.14$ & $4.18\pm0.65$ & Alt./Off.\\
\hline 
 3FGL J1748.3-2815c & 0.90 & -0.18 & 0.01 & 482.2 & 133.9 & $2.21\pm0.16$ & $0.66\pm0.24$ & $2.89\pm0.51$ & Alt./Off.\\
\hline 
 3FGL J1747.0-2828 & 0.37 & -0.06 & 0.01 & 2655.9 & 692.8 & $7.11\pm0.24$ & $0.48\pm0.13$ & $1.11\pm0.09$ & Alt./Off.\\
\hline 
 3FGL J1740.5-2843 & -0.44 & 1.02 & 0.04 & 142.7 & 48.6 & $0.82\pm0.11$ & $0.63\pm0.48$ & $1.48\pm0.50$ & Alt./Off.\\
\hline 
 3FGL J1747.7-2904 & 0.19 & -0.50 & 0.02 & 848.1 & 190.8 & $3.27\pm0.22$ & $0.80\pm0.23$ & $1.49\pm0.23$ & Alt./Off.\\
\hline 
 3FGL J1749.2-2911 & 0.11 & -0.80 & 0.04 & 173.9 & 78.7 & $1.01\pm0.13$ & $1.37\pm0.41$ & $1.68\pm0.56$ & Alt./Off.\\
\hline 
 3FGL J1754.0-2930 & 0.47 & -1.88 & 0.03 & 309.2 & 30.0 & $1.12\pm0.09$ & $1.72\pm0.29$ & $1.94\pm0.66$ & Alt./Off.\\
\hline 
 3FGL J1802.4-3043 & 0.31 & -4.03 & 0.02 & 120.1 & 101.2 & $0.27\pm0.04$ & $0.19\pm0.66$ & $3.20\pm1.07$ & Alt./Off.\\
\hline 
 3FGL J1820.4-3217 & 0.79 & -8.22 & 0.04 & 66.4 & 10.6 & $0.17\pm0.03$ & $0.54\pm0.77$ & $2.12\pm1.05$ & Alt./Off.\\
\hline 
 PS J1813.0-3145 & 0.48 & -6.52 & 0.04 & 64.5 & 20.4 & $0.16\pm0.03$ & $0.27\pm0.63$ & $2.60\pm1.03$ & Alt./Off.\\
\hline 
 3FGL J1830.8-3136 & 2.42 & -9.80 & 0.03 & 131.5 & 29.3 & $0.23\pm0.03$ & $0.90\pm0.40$ & $3.37\pm1.23$ & Alt./Off.\\
\hline 
 PS J1817.8-3334 & -0.64 & -8.26 & 0.05 & 81.6 & 17.7 & $0.21\pm0.03$ & $1.11\pm0.47$ & $1.94\pm0.78$ & Alt./Off.\\
\hline 
 PS J1839.1-3457 & 0.01 & -12.81 & 0.04 & 112.5 & 24.7 & $0.21\pm0.03$ & $1.40\pm0.33$ & $2.42\pm0.93$ & Alt./Off.\\
\hline 
 3FGL J1645.7-2149 & -1.84 & 15.01 & 0.05 & 90.7 & 15.7 & $0.27\pm0.04$ & $0.58\pm0.82$ & $0.78\pm0.38$ & Alt./Off.\\
\hline 
 PS J1656.6-2736 & -5.01 & 9.66 & 0.05 & 80.8 & 31.9 & $0.15\pm0.02$ & $0.35\pm0.90$ & $0.71\pm0.21$ & Alt./Off.\\
\hline 
 3FGL J1703.6-2850 & -5.06 & 7.69 & 0.04 & 60.3 & 11.6 & $0.18\pm0.03$ & $1.27\pm0.51$ & $4.23\pm2.32$ & Alt./Off.\\
\hline 
 PS J1711.1-3006 & -5.11 & 5.62 & 0.07 & 57.9 & 26.5 & $0.19\pm0.04$ & $0.19\pm0.71$ & $0.75\pm0.37$ & Alt./Off.\\
\hline 
 PS J1710.4-3035 & -5.64 & 5.44 & 0.07 & 32.1 & 14.4 & $0.12\pm0.03$ & $0.23\pm0.81$ & $1.25\pm0.92$ & Alt./Off.\\
\hline 
 3FGL J1734.7-2930 & -1.76 & 1.77 & 0.05 & 129.0 & 26.4 & $0.66\pm0.09$ & $0.98\pm0.61$ & $1.31\pm0.60$ & Alt./Off.\\
\hline 
 3FGL J1742.6-3321 & -4.10 & -1.68 & 0.02 & 304.1 & 31.6 & $1.01\pm0.09$ & $1.33\pm0.30$ & $2.05\pm0.58$ & Alt./Off.\\
\hline 
 PS J1736.2-3422 & -5.66 & -1.18 & 0.03 & 149.1 & 53.5 & $0.73\pm0.09$ & $1.56\pm0.32$ & $3.87\pm1.48$ & Alt./Off.\\
\hline 
 PS J1808.5-3523 & -3.21 & -7.40 & 0.06 & 36.3 & 16.3 & $0.09\pm0.02$ & $0.81\pm1.07$ & $1.45\pm0.78$ & Alt./Off.\\
\hline 
 3FGL J1808.3-3357 & -1.94 & -6.70 & 0.03 & 240.2 & 39.2 & $0.46\pm0.04$ & $1.23\pm0.33$ & $1.42\pm0.37$ & Alt./Off.\\
\hline 
 PS J1805.0-3620 & -4.39 & -7.23 & 0.05 & 86.2 & 27.1 & $0.19\pm0.03$ & $0.19\pm0.67$ & $1.42\pm0.57$ & Alt./Off.\\
\hline 
 3FGL J1808.4-3703 & -4.64 & -8.19 & 0.05 & 45.6 & 14.1 & $0.12\pm0.04$ & $0.16\pm0.42$ & $1.29\pm1.15$ & Alt./Off.\\
\hline 
 PS J1818.7-3203 & 0.71 & -7.75 & 0.09 & 55.0 & 16.4 & $0.17\pm0.04$ & $0.17\pm0.56$ & $0.90\pm0.49$ & Alt./Off.\\
\hline 
 3FGL J1641.5-2856 & -8.36 & 11.33 & 0.08 & 71.3 & 11.0 & $0.24\pm0.03$ & $1.83\pm0.46$ & $1.90\pm1.17$ & Alt./Off.\\
\hline 
 3FGL J1649.6-3007 & -8.01 & 9.21 & 0.02 & 238.4 & 40.0 & $0.37\pm0.04$ & $0.94\pm0.35$ & $2.22\pm0.62$ & Alt./Off.\\
\hline 
 PS J1643.4-3149 & -10.18 & 9.23 & 0.05 & 38.0 & 9.8 & $0.10\pm0.03$ & $0.14\pm0.30$ & $1.97\pm1.54$ & Alt./Off.\\
\hline 
 3FGL J1714.6-3327 & -7.34 & 3.00 & 0.04 & 101.5 & 19.3 & $0.35\pm0.07$ & $0.46\pm0.75$ & $1.65\pm0.85$ & Alt./Off.\\
\hline 
 3FGL J1726.6-3530c & -7.73 & -0.13 & 0.04 & 157.3 & 14.4 & $1.23\pm0.11$ & $1.92\pm0.21$ & $5.07\pm2.08$ & Alt./Off.\\
\hline 
\hline 
\end{tabular}
\caption{Best fit and uncertainty for the SED parameters of PSR 
  candidates derived with both the analysis performed with the 
  Official and Alternate IEM. The longitude, latitude, the $68\%$ 
  uncertainty for the position (pos\_68), $TS$, $TS^{\rm{PLE}}_{\rm{curv}}$ and the energy flux are also listed.}
\label{tab:psrcandrefoff}
\end{table*}

\begin{table*}
\center
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Name & l[deg]& b[deg] & pos\_68 & $TS$  & $TS^{\rm{PLE}}_{\rm{curv}}$  & $S$[$10^{-5}$MeV/cm$^2$/s] & $\Gamma$ & $E_{\rm{cutoff}}$ & IEM\\
\hline
\hline
 PS J1729.2-3502 & -7.02 & -0.34 & 0.02 & 121.9 & 18.0 & $0.87\pm0.14$ & $1.42\pm0.47$ & $4.58\pm2.40$ & Alt./Off.\\
\hline 
 PS J1731.4-3235 & -4.71 & 0.64 & 0.05 & 82.6 & 97.4 & $0.46\pm0.07$ & $0.14\pm0.84$ & $1.32\pm0.41$ & Alt./Off.\\
\hline 
 PS J1737.3-3334 & -4.83 & -0.95 & 0.06 & 42.4 & 75.4 & $0.35\pm0.07$ & $0.50\pm0.31$ & $0.62\pm0.27$ & Alt./Off.\\
\hline 
 3FGL J1748.5-3912 & -8.49 & -5.84 & 0.03 & 193.7 & 19.3 & $0.44\pm0.04$ & $1.61\pm0.28$ & $3.52\pm1.45$ & Alt./Off.\\
\hline 
 3FGL J1759.2-3848 & -7.15 & -7.41 & 0.03 & 165.9 & 28.0 & $0.30\pm0.04$ & $0.97\pm0.42$ & $2.20\pm0.70$ & Alt./Off.\\
\hline 
 3FGL J1656.9-3919c & -14.24 & 2.29 & 0.04 & 61.5 & 16.5 & $0.32\pm0.06$ & $1.41\pm0.42$ & $5.77\pm3.32$ & Alt./Off.\\
\hline 
 PS J1655.9-3940 & -14.64 & 2.27 & 0.05 & 60.9 & 19.9 & $0.31\pm0.06$ & $1.00\pm0.85$ & $2.42\pm2.05$ & Alt./Off.\\
\hline 
 PS J1721.7-3917 & -11.37 & -1.48 & 0.05 & 54.7 & 18.1 & $0.27\pm0.06$ & $0.31\pm0.61$ & $2.42\pm1.27$ & Alt./Off.\\
\hline 
 PS J1709.3-3943 & -13.06 & 0.11 & 0.07 & 83.0 & 13.8 & $0.87\pm0.12$ & $1.94\pm0.38$ & $3.09\pm1.70$ & Alt./Off.\\
\hline 
 PS J1744.0-4323 & -12.56 & -7.20 & 0.07 & 52.5 & 24.6 & $0.12\pm0.02$ & $0.89\pm0.63$ & $1.29\pm0.70$ & Alt./Off.\\
\hline 
 3FGL J1753.6-4447 & -12.93 & -9.36 & 0.03 & 265.9 & 25.7 & $0.39\pm0.04$ & $1.34\pm0.28$ & $2.67\pm0.88$ & Alt./Off.\\
\hline 
 3FGL J1823.2-4722 & -12.87 & -15.09 & 0.04 & 86.6 & 25.4 & $0.13\pm0.02$ & $0.58\pm0.66$ & $1.97\pm0.85$ & Alt./Off.\\
\hline 
 3FGL J1624.2-3957 & -18.81 & 6.67 & 0.03 & 121.1 & 19.1 & $0.26\pm0.05$ & $0.56\pm0.71$ & $2.42\pm1.03$ & Alt./Off.\\
\hline 
 3FGL J1652.8-4351 & -18.29 & 0.08 & 0.03 & 439.8 & 73.7 & $2.15\pm0.13$ & $1.58\pm0.19$ & $2.20\pm0.49$ & Alt./Off.\\
\hline 
 PS J1830.0-5226 & -17.38 & -18.11 & 0.05 & 50.0 & 11.1 & $0.08\pm0.02$ & $0.08\pm0.44$ & $2.26\pm1.24$ & Alt./Off.\\
\hline 
 3FGL J1824.2-5427 & -19.68 & -18.05 & 0.03 & 129.6 & 22.6 & $0.15\pm0.02$ & $0.58\pm0.47$ & $2.46\pm0.89$ & Alt./Off.\\
\hline 
 PS J1730.0-3422 & -6.37 & -0.13 & 0.05 & 42.6 & 10.7 & $0.59\pm0.13$ & $1.03\pm0.77$ & $1.34\pm0.74$ & Alt./Off.\\
\hline
\hline
\end{tabular}
\caption{Continuation of Tab.~\ref{tab:psrcandrefoff}}
\label{tab:psrcandrefoffcont}
\end{table*}




\begin{table*}
\center
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Name & l[deg]& b[deg] & pos\_68 & $TS$  & $TS^{\rm{PLE}}_{\rm{curv}}$  & IEM & ATNF & $P$[s] & dist[deg]\\
\hline
\hline
 3FGL J1823.2-1339 & 17.59 & -0.10 & 0.01 & 1287.3 & 58.6 & $4.33\pm0.19$ & $1.99\pm0.08$ & $8.62\pm1.80$ & Off. \\
\hline 
 PS J1828.2-1312 & 18.53 & -0.92 & 0.06 & 44.8 & 28.6 & $0.41\pm0.09$ & $1.38\pm0.74$ & $0.62\pm0.14$ & Off. \\
\hline 
 3FGL J1829.7-1304 & 18.88 & -1.05 & 0.06 & 60.6 & 26.5 & $0.46\pm0.08$ & $0.69\pm0.46$ & $1.11\pm0.44$ & Off. \\
\hline 
 3FGL J1806.7-2451 & 5.93 & -2.05 & 0.06 & 55.0 & 96.6 & $0.36\pm0.07$ & $0.09\pm0.47$ & $0.78\pm0.46$ & Off. \\
\hline 
 3FGL J1744.5-2506 & 3.19 & 2.06 & 0.09 & 70.8 & 239.2 & $0.51\pm0.09$ & $1.69\pm0.70$ & $1.70\pm1.16$ & Off. \\
\hline 
 3FGL J1737.9-2511 & 2.36 & 3.38 & 0.04 & 207.1 & 17.8 & $0.80\pm0.07$ & $1.77\pm0.39$ & $1.52\pm0.71$ & Off. \\
\hline 
 3FGL J1740.5-2642 & 1.32 & 2.14 & 0.04 & 178.4 & 28.6 & $0.77\pm0.08$ & $1.50\pm0.34$ & $2.04\pm0.69$ & Off. \\
\hline 
 3FGL J1736.5-2839 & -0.86 & 1.88 & 0.09 & 111.4 & 20.7 & $0.65\pm0.11$ & $0.23\pm0.97$ & $0.43\pm0.14$ & Off. \\
\hline 
 PS J1824.9-3244 & 0.73 & -9.21 & 0.08 & 34.2 & 9.7 & $0.11\pm0.03$ & $0.28\pm0.66$ & $1.77\pm1.20$ & Off. \\
\hline 
 PS J1702.3-2527 & -2.50 & 9.92 & 0.04 & 49.5 & 9.2 & $0.13\pm0.03$ & $0.84\pm0.53$ & $7.11\pm3.75$ & Off. \\
\hline 
 3FGL J1739.9-3124c & -2.53 & -0.41 & 0.07 & 59.4 & 81.5 & $0.75\pm0.17$ & $1.88\pm0.43$ & $5.74\pm4.16$ & Off. \\
\hline 
 PS J1743.9-2860 & -0.23 & 0.20 & 0.04 & 463.1 & 281.8 & $2.34\pm0.16$ & $0.72\pm0.63$ & $0.90\pm0.30$ & Off. \\
\hline 
 PS J1823.8-3544 & -2.06 & -10.33 & 0.05 & 37.3 & 16.5 & $0.10\pm0.03$ & $0.93\pm0.85$ & $3.00\pm2.17$ & Off. \\
\hline 
 PS J1858.6-4447 & -8.06 & -19.94 & 0.07 & 37.0 & 9.9 & $0.09\pm0.02$ & $1.56\pm0.80$ & $2.90\pm2.16$ & Off. \\
\hline 
 PS J1705.5-3852 & -12.87 & 1.31 & 0.06 & 35.4 & 26.5 & $0.18\pm0.04$ & $1.21\pm0.69$ & $1.24\pm0.61$ & Off. \\
\hline 
 PS J1652.1-4430 & -18.84 & -0.22 & 0.04 & 60.1 & 31.4 & $0.75\pm0.21$ & $1.59\pm0.56$ & $3.03\pm2.05$ & Off. \\
\hline 
 3FGL J1733.5-2811 & -0.66 & 2.45 & 0.07 & 151.4 & 59.8 & $0.75\pm0.14$ & $1.56\pm0.90$ & $1.02\pm0.72$ & Off. \\
\hline 
 3FGL J1705.5-4128c & -15.07 & -0.31 & 0.13 & 28.4 & 144.2 & $0.47\pm0.16$ & $1.73\pm0.93$ & $3.67\pm2.26$ & Off. \\
\hline 
 3FGL J1650.0-4438c & -19.30 & 0.04 & 0.04 & 65.9 & 18.4 & $0.58\pm0.11$ & $0.96\pm0.59$ & $4.09\pm2.19$ & Off. \\
\hline 
 PS J1652.1-4430 & -18.77 & 0.02 & 0.05 & 105.3 & 35.1 & $1.10\pm0.17$ & $1.95\pm0.45$ & $3.44\pm2.63$ & Off. \\
\hline 
\hline 
\end{tabular}
\caption{Same as in Tab.~\ref{tab:psrcandrefoff} but for the PSR candidates found only for the analysis where the Official IEM is considered.}
\label{tab:psrcandoff}
\end{table*}


\begin{table*}
\center
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Name & l[deg]& b[deg] & pos\_68 & $TS$  & $TS^{\rm{PLE}}_{\rm{curv}}$  & $S$[$10^{-5}$MeV/cm$^2$/s] & $\Gamma$ & $E_{\rm{cutoff}}$ & IEM\\
\hline
\hline
  3FGL J1819.5-1345 & 17.13 & 0.75 & 0.05 & 184.4 & 108.8 & $1.19\pm0.14$ & $1.45\pm0.36$ & $1.47\pm0.46$ & Alt. \\
\hline 
 PS J1739.2-1101 & 14.61 & 10.66 & 0.10 & 32.4 & 24.3 & $0.16\pm0.08$ & $0.62\pm0.71$ & $1.02\pm0.43$ & Alt. \\
\hline 
 3FGL J1814.0-1757c & 12.75 & 0.01 & 0.03 & 124.5 & 27.7 & $1.15\pm0.18$ & $1.72\pm0.25$ & $9.13\pm5.19$ & Alt. \\
\hline 
 PS J1811.7-1840 & 11.83 & 0.01 & 0.03 & 220.5 & 25.9 & $1.46\pm0.16$ & $1.11\pm0.42$ & $1.26\pm0.41$ & Alt. \\
\hline 
 PS J1818.5-1654 & 14.19 & -0.61 & 0.03 & 85.2 & 99.7 & $0.79\pm0.12$ & $1.35\pm0.37$ & $3.72\pm1.60$ & Alt. \\
\hline 
 PS J1836.5-2401 & 9.81 & -7.63 & 0.07 & 45.0 & 18.3 & $0.18\pm0.04$ & $1.37\pm0.60$ & $2.59\pm1.60$ & Alt. \\
\hline 
 PS J1759.8-2354 & 5.93 & -0.14 & 0.04 & 302.1 & 460.3 & $1.89\pm0.23$ & $1.72\pm0.18$ & $8.36\pm2.83$ & Alt. \\
\hline 
 3FGL J1758.8-2346 & 6.03 & 0.23 & 0.03 & 204.1 & 33.9 & $1.31\pm0.15$ & $1.64\pm0.25$ & $9.31\pm5.79$ & Alt. \\
\hline 
 3FGL J1729.7-2408 & 2.25 & 5.56 & 0.05 & 65.9 & 30.6 & $0.25\pm0.04$ & $0.20\pm0.81$ & $0.53\pm0.17$ & Alt. \\
\hline 
 PS J1739.3-2829 & -0.38 & 1.42 & 0.06 & 56.9 & 20.6 & $0.38\pm0.12$ & $0.52\pm 0.23$ & $1.79\pm1.08$ & Alt. \\
\hline 
 PS J1740.5-2908 & -0.78 & 0.85 & 0.04 & 112.1 & 23.1 & $0.88\pm0.12$ & $1.50\pm0.41$ & $3.13\pm1.80$ & Alt. \\
\hline 
 PS J1758.3-3028 & 0.09 & -3.16 & 0.03 & 64.8 & 82.2 & $0.27\pm0.05$ & $0.81\pm0.82$ & $2.46\pm1.90$ & Alt. \\
\hline 
 PS J1744.7-2922 & -0.40 & -0.07 & 0.03 & 535.2 & 251.0 & $2.71\pm0.17$ & $0.36\pm0.42$ & $0.95\pm0.14$ & Alt. \\
\hline 
 PS J1747.9-3015 & -0.85 & -1.08 & 0.04 & 61.8 & 16.6 & $0.57\pm0.11$ & $1.40\pm0.29$ & $8.76\pm3.49$ & Alt. \\
\hline 
 PS J1735.6-3219 & -4.01 & 0.04 & 0.04 & 57.8 & 555.0 & $0.56\pm0.12$ & $1.03\pm0.55$ & $3.38\pm1.71$ & Alt. \\
\hline 
 PS J1750.1-2855 & 0.63 & -0.86 & 0.07 & 68.1 & 29.8 & $0.55\pm0.13$ & $0.08\pm 0.68$ & $1.09\pm0.97$ & Alt. \\
\hline 
 3FGL J1628.2-2431c & -6.87 & 16.53 & 0.07 & 82.7 & 14.5 & $0.41\pm0.08$ & $1.66\pm0.40$ & $2.74\pm1.63$ & Alt. \\
\hline 
 PS J1632.2-2352 & -5.65 & 16.29 & 0.06 & 54.5 & 13.9 & $0.24\pm0.05$ & $1.45\pm0.61$ & $3.00\pm2.34$ & Alt. \\
\hline 
 PS J1632.7-2435 & -6.06 & 15.72 & 0.06 & 50.0 & 20.8 & $0.21\pm0.04$ & $0.54\pm0.66$ & $1.65\pm0.84$ & Alt. \\
\hline 
 3FGL J1747.0-3506 & -5.16 & -3.44 & 0.08 & 40.2 & 12.4 & $0.19\pm0.05$ & $1.86\pm0.76$ & $3.01\pm1.40$ & Alt. \\
\hline 
 3FGL J1758.8-4108 & -9.22 & -8.49 & 0.02 & 166.6 & 10.3 & $0.34\pm0.04$ & $1.92\pm0.19$ & $9.50\pm4.68$ & Alt. \\
\hline 
 PS J1653.9-3509 & -11.37 & 5.40 & 0.04 & 47.8 & 11.4 & $0.20\pm0.04$ & $1.54\pm0.37$ & $8.24\pm4.85$ & Alt. \\
\hline 
 3FGL J1700.4-4019c & -14.56 & 1.27 & 0.05 & 72.7 & 31.7 & $0.41\pm0.32$ & $1.66\pm 0.51$ & $6.11\pm4.26$ & Alt. \\
\hline 
 PS J1705.3-4030 & -14.25 & 0.38 & 0.02 & 323.0 & 33.2 & $1.63\pm0.14$ & $1.78\pm0.18$ & $5.83\pm1.93$ & Alt. \\
\hline 
 3FGL J1717.6-4404 & -15.70 & -3.55 & 0.08 & 25.4 & 9.6 & $0.19\pm0.06$ & $1.27\pm0.65$ & $3.38\pm5.43$ & Alt. \\
\hline 
 PS J1808.2-4519 & -12.16 & -11.93 & 0.07 & 31.6 & 22.1 & $0.09\pm0.02$ & $0.61\pm0.96$ & $1.93\pm1.16$ & Alt. \\
\hline 
 3FGL J1813.6-1148 & 18.43 & 3.03 & 0.05 & 146.2 & 10.8 & $0.72\pm0.10$ & $1.82\pm0.41$ & $3.25\pm2.16$ & Alt. \\
\hline 
 PS J1817.3-1342 & 16.88 & 0.90 & 0.09 & 67.3 & 68.3 & $0.67\pm0.14$ & $1.61\pm0.47$ & $2.38\pm1.32$ & Alt. \\
\hline 
 PS J1825.6-1218 & 19.05 & -0.00 & 0.06 & 83.5 & 25.7 & $0.99\pm0.17$ & $1.30\pm0.63$ & $2.12\pm1.42$ & Alt. \\
\hline 
 PS J1820.6-1450 & 16.19 & -0.10 & 0.06 & 136.8 & 75.8 & $1.25\pm0.20$ & $1.14\pm 0.44$ & $0.96\pm0.88$ & Alt. \\
\hline 
 PS J1840.4-1707 & 16.42 & -5.35 & 0.05 & 42.9 & 10.5 & $0.13\pm0.03$ & $0.65\pm0.49$ & $1.11\pm0.58$ & Alt. \\
\hline 
 PS J1839.2-1504 & 18.13 & -4.16 & 0.07 & 35.3 & 11.4 & $0.14\pm0.04$ & $0.66\pm0.97$ & $2.63\pm1.50$ & Alt. \\
\hline 
 PS J1814.2-1713 & 13.42 & 0.19 & 0.04 & 108.2 & 21.2 & $1.00\pm0.17$ & $0.68\pm0.97$ & $1.00\pm0.61$ & Alt. \\
\hline 
 PS J1817.4-1617 & 14.63 & -0.10 & 0.05 & 205.9 & 94.1 & $1.61\pm0.17$ & $1.48\pm0.61$ & $0.93\pm0.48$ & Alt. \\
\hline 
 PS J1743.4-1825 & 8.70 & 5.90 & 0.10 & 47.1 & 23.8 & $0.18\pm0.03$ & $0.80\pm0.31$ & $0.87\pm0.42$ & Alt. \\
\hline 
 PS J1750.5-1907 & 9.00 & 4.12 & 0.07 & 37.3 & 27.5 & $0.19\pm0.05$ & $0.75\pm0.50$ & $2.12\pm1.28$ & Alt. \\
\hline 
 PS J1801.8-2245 & 7.10 & 0.03 & 0.06 & 91.3 & 70.2 & $1.00\pm0.18$ & $1.82\pm0.51$ & $5.16\pm3.25$ & Alt. \\
\hline 
 PS J1756.8-2433 & 4.99 & 0.07 & 0.05 & 119.8 & 44.7 & $0.75\pm0.10$ & $0.64\pm0.35$ & $0.81\pm0.48$ & Alt. \\
\hline 
 PS J1837.7-2902 & 5.35 & -10.14 & 0.10 & 39.9 & 12.1 & $0.13\pm0.03$ & $0.54\pm0.89$ & $1.10\pm0.57$ & Alt. \\
\hline 
 PS J1740.6-2807 & 0.21 & 1.40 & 0.05 & 88.9 & 9.2 & $0.69\pm0.13$ & $1.72\pm0.69$ & $1.97\pm1.44$ & Alt. \\
\hline 
 3FGL J1800.0-2955 & 0.75 & -3.22 & nan & 37.9 & 116.3 & $0.19\pm0.04$ & $0.98\pm0.34$ & $0.39\pm0.06$ & Alt. \\
\hline 
 PS J1752.7-2845 & 0.96 & -1.18 & 0.06 & 85.6 & 37.5 & $0.50\pm0.10$ & $0.35\pm0.33$ & $1.30\pm0.78$ & Alt. \\
\hline 
 PS J1752.4-3001 & -0.18 & -1.80 & 0.06 & 61.7 & 9.4 & $0.44\pm0.13$ & $1.34\pm0.59$ & $2.06\pm1.24$ & Alt. \\
\hline 
 PS J1747.4-2809 & 0.98 & 0.06 & 0.03 & 97.4 & 19.9 & $0.99\pm0.18$ & $1.11\pm0.43$ & $4.06\pm1.56$ & Alt. \\
\hline 
 PS J1750.8-3025 & -0.65 & -1.73 & 0.07 & 40.4 & 15.7 & $0.35\pm0.09$ & $1.05\pm0.88$ & $1.79\pm1.30$ & Alt. \\
\hline 
 PS J1723.0-2902 & -2.68 & 4.18 & 0.11 & 39.9 & 9.1 & $0.22\pm0.06$ & $0.35\pm0.66$ & $0.64\pm0.42$ & Alt. \\
\hline 
 PS J1732.7-2903 & -1.59 & 2.26 & 0.10 & 49.5 & 46.6 & $0.38\pm0.09$ & $1.63\pm0.61$ & $4.11\pm3.03$ & Alt. \\
\hline 
 PS J1735.7-3025 & -2.39 & 1.02 & 0.04 & 208.2 & 88.6 & $0.81\pm0.09$ & $0.22\pm0.60$ & $1.03\pm0.26$ & Alt. \\
\hline 
 PS J1734.6-3237 & -4.41 & 0.03 & 0.06 & 69.3 & 79.5 & $0.65\pm0.11$ & $1.15\pm0.42$ & $3.36\pm1.40$ & Alt. \\
\hline 
 PS J1750.1-2855 & 0.55 & -0.64 & 0.08 & 75.5 & 32.7 & $0.75\pm0.15$ & $0.67\pm0.41$ & $1.50\pm1.18$ & Alt. \\
\hline 
 PS J1711.1-3922 & -12.81 & 0.05 & 0.05 & 116.6 & 24.0 & $0.78\pm0.14$ & $0.57\pm0.76$ & $1.46\pm0.66$ & Alt. \\
\hline 
 PS J1720.5-3710 & -9.74 & -0.04 & 0.05 & 122.2 & 22.4 & $0.97\pm0.14$ & $1.20\pm0.55$ & $1.55\pm0.67$ & Alt. \\
\hline 
 PS J1707.5-4028 & -13.92 & 0.04 & 0.04 & 175.4 & 24.8 & $1.18\pm0.15$ & $1.36\pm0.41$ & $1.82\pm0.71$ & Alt. \\
\hline 
 PS J1627.8-3854 & -17.66 & 6.88 & 0.06 & 31.7 & 9.4 & $0.13\pm0.04$ & $0.72\pm0.22$ & $2.77\pm1.66$ & Alt. \\
\hline 
 3FGL J1705.5-4128c & -14.88 & -0.21 & 0.08 & 163.0 & 11.5 & $1.14\pm0.15$ & $1.49\pm0.45$ & $2.25\pm1.19$ & Alt. \\
\hline 
\hline 
\end{tabular}
\caption{Same as in Tab.~\ref{tab:psrcandoff} but for the PSR candidates found only for the analysis where the Alternate IEM is considered.}
\label{tab:psrcandref1}
\end{table*}





